Footnotes to the birational geometry of primitive symplectic varieties

In this note, we extend to the singular case some results on the birational geometry of irreducible holomorphic symplectic manifolds.

==> preamble.tex <==
\renewcommand{\baselinestretch}{1.25} 
\usepackage{anysize} \marginsize{1.3in}{1.3in}{1in}{1in}

\usepackage{xcolor}
\usepackage{amsmath}

\makeatletter
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{%
  \begingroup
  \def\mathaccent##1##2{%
    \rel@kern{0.8}%
    \overline{\rel@kern{-0.8}\macc@nucleus\rel@kern{0.2}}%
    \rel@kern{-0.2}%
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \macc@nested@a\relax111{#1}%
  \endgroup
}

\usepackage{mathtools}
\usepackage[all]{xy}
\usepackage[utf8]{inputenc}
%\usepackage[latin1]{inputenc}
\usepackage{varioref}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{xparse}
%\usepackage{showkeys}
%\usepackage[notcite, notref]{showkeys}
\usepackage{graphicx}
\usepackage{mathrsfs}
\usepackage[hypertexnames=false,backref=page,pdftex,
 	pdfpagemode=UseNone,
 	breaklinks=true,
 	extension=pdf,
 	colorlinks=true,
 	linkcolor=blue,
 	citecolor=red,
 	urlcolor=blue,
 ]{hyperref}
\renewcommand*{\backref}[1]{{-- cited on p.~#1}}

